The Effect of Masking Strategies on Knowledge Retention by Language Models

Language models retain a significant amount of world knowledge from their pre-training stage. This allows knowledgeable models to be applied to knowledge-intensive tasks prevalent in information retrieval, such as ranking or question answering. Understanding how and which factual information is acquired by our models is necessary to build responsible models. However, limited work has been done to understand the effect of pre-training tasks on the amount of knowledge captured and forgotten by language models during pre-training. Building a better understanding of knowledge acquisition is the goal of this paper. Therefore, we utilize a selection of pre-training tasks to infuse knowledge into our model. In the following steps, we test the model's knowledge retention by measuring its ability to answer factual questions. Our experiments show that masking entities and principled masking of correlated spans based on pointwise mutual information lead to more factual knowledge being retained than masking random tokens. Our findings demonstrate that, like the ability to perform a task, the (factual) knowledge acquired from being trained on that task is forgotten when a model is trained to perform another task (catastrophic forgetting) and how to prevent this phenomenon. To foster reproducibility, the code, as well as the data used in this paper, are openly available.

==> chapters/experiments_old.tex <==
\section{Experiments}

% We train all models on CBQA. Some models are first exposed to additional pre-training.

% \subsection{Hyperparameters}
% Tianyi please fill details of the used models and training. Batch size, any other details you might have used when training 

\subsection{Data}
We use the PAQ dataset \citep{DBLP:journals/corr/LewisPAQ} for our experiments. This dataset contains a set of 65M QA pairs automatically generated from Wikipedia passages. Since the QA pairs are derived from a passage, we can be sure that the question's answer can be found in the said passage. This property makes this dataset relevant for our research into how facts are acquired from textual corpi. To keep our experiments tractable, we select 10K passages from the full PAQ dataset, with each passage containing four or more QA pairs. For the additional pretraining, we utilize the full 10K passages, which we will refer to as PAQ-passages. For the CBQA training, we split the ~49k QA pairs into train (76\%), dev (10\%), and test sets (14\%). 
% An overview of the dataset can be found in Table~\ref{tab:dataset}.

% \begin{table*}[]
% \centering
% \begin{tabular}{lllll}
%     & \textbf{\#Passages} & \textbf{\#CBQA-train} & \textbf{\#CBQA-dev} & \textbf{\#CBQA-test} \\ \hline
% PAQ & 10.000              & 37.181                & 5.000               & 7.000                 \\ \hline
% \end{tabular}
% \caption{Subset of the full PAQ65M dataset used in the experiments.}
% \label{tab:dataset}
% \end{table*}

\subsection{Results}

Given the previously established methodology and data, we report our findings in this section. 

\mpara{Random masking is least effective for retaining knowledge.}
First, we experiment with the three different masking strategies on the PAQ dataset. We followed the methodology depicted in Figure~\ref{fig:experimental_setup}: Pretraining on the PAQ Wikipedia passages with one of our three pretraining tasks, followed by CBQA fine-tuning on the training set of corresponding QA pairs. Lastly, we measure the amount of knowledge retained from pretraining by the difference to a baseline model that was not additionally pretrained. All experiments are repeated four times.
The results are reported in Figure~\ref{fig:pt_standard_setting}. First of all, we find the process of additional pretraining to improve the amount of knowledge retained for the downstream task, no matter of the specific masking strategy. This is in line with other works, reporting that additional pretraining improves the CBQA performance \citep{DBLP:journals/corr/GuuREALM, DBLP:conf/emnlp/RobertsRS20, DBLP:journals/corr/LewisPAQ}. Next, we observe PMI masking and SSM to outperform masking random tokens. We hypothize that this is the case, because RTM results in many easy to guess examples being masked (see Section~\ref{sec:infusing_knowledge}). Facts - or relational knowledge - are often expressed in the interactions and context of entities. However, by masking easy-to-guess examples, the model is never required to understand the broader context in which entities appear. Last, while we find the average performance of SSM and PMI to be fairly similar, we observe less variance between runs with PMI masking compared to SSM or RTM.

% \begin{figure*}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/tmp/results_F1.pdf}
%     \caption{CBQA performance in F1 score for the baseline without additional pretraining (i.e., only fine-tuning, FT) and three models with additional pretraining and different masking strategies (RTM, SSM, PMI masking).}
%     \label{fig:pt_standard_setting}
% \end{figure*}

% \begin{figure}[ht]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/tmp/results_EM.pdf}
%     \caption{CBQA performance in EM score for the baseline without additional pretraining (i.e., only fine-tuning, FT) and three models with additional pretraining and different masking strategies (RTM, SSM, PMI masking).}
%     \label{fig:pt_standard_setting_EM}
% \end{figure}

\begin{figure*}[ht]
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/tmp/results_F1.pdf}
%   \caption{F1 Score}
%   \label{fig:sfig1}
\end{subfigure}
\begin{subfigure}{.48\textwidth}
  \centering
  \includegraphics[width=.99\linewidth]{figures/tmp/results_EM.pdf}
%   \caption{Exact Match}
%   \label{fig:sfig2}
\end{subfigure}
\caption{CBQA performance in F1 and EM score for the baseline without additional pretraining (i.e., only fine-tuning, FT) and three models with additional pretraining and different masking strategies (RTM, SSM, PMI masking - PT + FT). Additionally, the effect of elastic weight consolidation (EWC), multi-task learning PT objective and CBQA in parallel (MTL) and MTL followed by another round of fine-tuning (MTL + FT)}
\label{fig:results_big}
\end{figure*}


% \begin{figure}[h!]
%     \centering
%     \includegraphics[width=0.34\textwidth]{updated_plots/bert/multi_mean_P_AT_1.png}
%     \caption{Mean P@1 of \bert{} across all layers.}
%     \label{fig:bert_layers}
% \end{figure}

\mpara{The sequential learning problem applies to factual knowledge.}
% Show that catastrophic forgetting is a problem
Interestingly, the additional pretraining step on knowledge-rich textual data usually leads to small improvements in CBQA performance - typically a few percent in F1 or exact match \citep{DBLP:journals/corr/LewisPAQ, DBLP:journals/corr/GuuREALM}. This is what we observe in Figure~\ref{fig:pt_standard_setting}, despite a intensive additional pretraining stage on passages that we can be sure to contain the factual information (other than REALM, which tries to retrieve useful information from a corpus \citep{DBLP:journals/corr/GuuREALM}). Thus, we wonder if the sequential learning problem (also referred to as catastrophic forgetting) applies to the factual knowledge being stored in the model's parametric memory. 
% Short description of what I call catastrophic forgetting in this setting
The classical sequential learning problem occurs when a model is trained on an initial task, fine-tuned on another, and required to perform the initial again. In this scenario, many works have shown that the model is likely to (partially) lose its ability to perform the initial task \citep{McCloskey1989CatastrophicII}. Here, we hypothize that this also applies to the (factual) knowledge acquired with the first task \todo{(might also partially explain why fine-tuned models were performing bad in knowledge tasks in \citep{wallat-etal-2020-bertnesia})}. Therefore, we will experiment with common approaches to counter the sequential learning problem.  

% 

\mpara{Elastic Weight Consolidation.}
In the first set of experiments, we additionally pretrained our models on the three tasks as before, but use the elastic weight consolidation regularizer (EWC, \citep{DBLP:journals/corr/KirkpatrickPRVD16}) in the fine-tuning stage. As EWC tries to preserve weights that are important for the initial task, it might also preserve the world knowledge acquired with this task. 

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/ewc.png}
%     \caption{F1 Score comparing the training w/o EWC and /w EWC.}
%     \label{fig:pt_ewc}
% \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/tmp/ewc_mtl.png}
%     \caption{F1 Score comparing the training with EWC/MTL to the standard pretraining and fine-tuning setup.}
%     \label{fig:pt_ewc}
% \end{figure}

Figure~\ref{fig:pt_ewc} compares the F1 scores achieved by the pretraining tasks with and without EWC. It is directly evident that the amount of knowledge being retained and usable from the pretraining stage is vastly increased with the usage of EWC. This suggests that the problem of catastrophic forgetting indeed applies to the knowledge captured from an initial task. In these experiments with EWC, we again find SSM and PMI masking to outperform RTM. However, the differences between the masking strategies are not as striking as in the standard setting. Additionally, a benefit of EWC is a reduced amount of variance between runs with the same masking strategy.  



\mpara{Multi-task Learning.}
Given the success of EWC to counter the forgetting of factual knowledge, we next experiment with multi-task learning. MTL has been shown to work well regarding retaining the ability to perform multiple tasks \citep{DBLP:conf/gcai/RibeiroMD19}. By not training two tasks sequentially, MTL forces to model to keep the ability to perform well in both tasks at the same time. Thus, we compare our standard setup with two different training strategies: Multi-task training both the additional pretraining and the CBQA fine-tuning together as well as the aforementioned Multi-task setup, followed by an additional CBQA fine-tuning step. The results are shown in Figure~\ref{fig:pt_multitask}.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/multitask.png}
%     \caption{F1 for the multitask setting.}
%     \label{fig:pt_multitask}
% \end{figure}

Similar to EWC, we found MTL to outperform the common setting of additional pretraining followed by CBQA fine-tuning. The standard MTL setup performs similarly to EWC, however, these results can be further improved by another round of fine-tuning. With this additional round of fine-tuning, we also observe the least amount of performance variance.


==> chapters/into_old.tex <==
\section{Introduction}


% What
% 
Over recent years, machine learning models have been increasingly applied to knowledge intensive tasks \citep{DBLP:conf/naacl/PetroniPFLYCTJK21}; question answering, ranking, and fact checking, to name only a few. Besides their training objectives, one goal of these models is to retain as much factual knowledge as possible from the training stage. Closed-book question answering (CBQA) \citep{DBLP:conf/nips/LewisPPPKGKLYR020} is one of these knowledge-intense tasks, which requires the model to produce an answer only from its parametric memory after being prompted a question. 

% No pretraining in the first paragraph
To improve the amount of knowledge stored in the model's parametric memory, recent studies \citep{DBLP:journals/corr/LewisPAQ, DBLP:conf/emnlp/RobertsRS20} applied a second stage of pretraining (from here on referred to as \textit{additional pretraining}). In the additional pretraining setting, the model is continued to be trained on a corpus deemed to contain a high amount of relevant information with the goal to capture as much knowledge as possible. For the training objective, most studies default to the model's standard language modeling tasks or tasks found to be useful with retriever models \citep{DBLP:journals/corr/GuuREALM, DBLP:conf/emnlp/RobertsRS20, DBLP:journals/corr/LewisPAQ}. In this study, we aim to shed more light on the effectiveness and pitfalls of the additional pretraining stage. 

% \begin{figure}
%     \centering
%     \includegraphics[width=0.49\textwidth]{figures/knowledge_pt_method_larger.pdf}
%     \caption{Experimental setup. First the model is additionally pretrained on knowledge-intense passages from Wikipedia, then it is trained on closed-book question answering and tested to measure the amount of knowledge retained.}
%     \label{fig:experimental_setup}
% \end{figure}

\begin{figure*}
    \centering
    \includegraphics[width=0.8\textwidth]{figures/knowledge_pt_method_wide.drawio.pdf}
    \caption{Experimental setup. First the model is additionally pretrained on knowledge-intense passages from Wikipedia, then it is trained on closed-book question answering and tested to measure the amount of knowledge retained.}
    \label{fig:experimental_setup}
\end{figure*}

% Why
% A better grasp of knowledge retention will allow us to build more knowledge models. 
A better grasp of how knowledge is acquired and retained for downstream tasks could yield two major benefits: First, it will allow us to build more knowledge intensive models, enabling better task performance for tasks such as CBQA. Second, it will be an early step in understanding when and under which circumstances unwanted or biased knowledge might be retained, potentially allowing us to later build more robust, socially responsible models.
% Limitations
Other studies successfully applied additional pretraining with the primary goal to achieve SotA CBQA performance. However, a systematic analysis of additional pretraining, its tasks, and paradigms has - to the best of our knowledge - not yet been conducted. 

\todo{Mention probing}
% Our solution/idea
To understand how knowledge is retained from the additional pretraining stage and applied in CBQA, we leverage the PAQ dataset \citep{DBLP:journals/corr/LewisPAQ} which contains Wikipedia passages and a set of question-answer pairs derived from that passage. This direct relation between a pretraining corpus and CBQA dataset allows for a systematic investigation of different pretraining tasks and their effect on the amount of factual knowledge being retained. Therefore, we devise a three-step process (see Figure~\ref{fig:experimental_setup}): Firstly, a T5 model \citep{DBLP:journals/jmlr/RaffelSRLNMZLL20} is additionally pretrained on the PAQ Wikipedia passages to capture relevant knowledge. Secondly, the model is trained for CBQA on a subset of the aligned QA pairs and lastly, we measure the amount of factual knowledge retained from training on a hold-out CBQA test set. In our study, we experiment with span corruption (RTM, random token masking - T5's version of language modeling) \citep{DBLP:journals/jmlr/RaffelSRLNMZLL20}, salient span masking (SSM, masking entities) \citep{DBLP:conf/acl/ZhangHLJSL19}, and PMI masking (masking by the pointwise mutual information of sequences) \citep{DBLP:conf/iclr/LevineLLALTS21}. 

% Experiments and some highlight results
While we find that all additional pretraining tasks improve the amount of knowledge captured, SSM and PMI masking seem to be more effective than masking random tokens. Furthermore, our experiments suggest that catastrophic forgetting also occurs with factual knowledge and that these effects can be mitigated by regularization strategies such as elastic weight consolidation (EWC) \citep{DBLP:journals/corr/KirkpatrickPRVD16} or multi-task learning (MTL). 

% Contributions
\subsection{Contributions}
% Our research question and how it is novel
The fact that language models acquire factual knowledge from their pretraining is widely accepted and utilized for applying LMs to knowledge intensive tasks. Yet, it is poorly understood how and which knowledge is retained from training. Therefore, we pose two research questions: \textit{RQ1: "What is the effect of pretraining tasks on the amount of knowledge being acquired?"} and \textit{RQ2: "Is this knowledge still usable after fine-tuning for downstream tasks?"}


% Our approach
This study aims to improve our understanding of the parametric memory, by systematically studying the effect of additional pretraining tasks on the amount of factual knowledge captured and retained by the model. We utilize Wikipedia passages and corresponding QA pairs to first training the model on the passages and later testing the amount of knowledge captured via the QA pairs. The procedure is depicted Figure~\ref{fig:experimental_setup}. Our key findings summarize as follows:

\mpara{Pretraining tasks.} While we show that all tasks result in the model retaining factual knowledge from the additional pretraining corpus, both average performance and variance vary from task to task. Our results suggest that SSM and PMI masking both outperform random token masking (61.1\%), with PMI masking having the least amount of variance between runs (72.0\% compared to others \%). 

\mpara{Catastrophic forgetting of knowledge.} We show that the sequential learning problem also occurs with the current training paradigm of additional pretraining followed by closed-book question answering. This is in line with the findings of \citet{wallat-etal-2020-bertnesia}, who observed that fine-tuning leads to factual knowledge being forgotten.

\mpara{Mitigation of catastrophic forgetting.} We find that common countermeasures to catastrophic forgetting can be applied to mitigate the effect of knowledge no longer being accessible. Multi-task learning seems to be slightly more effective than elastic weight consolidation (EWC), yet both result in significant performance improvement over the baseline. Additionally, we find that MTL and EWC reduce the run performance variance by XYZ and WXY\%.

% Key findings

% To improve our understanding of the parametric memory, we systematically study the effect of additional pretraining tasks on the amount of factual knowledge captured and retained by the model. Therefore, we utilize knowledge-dense Wikipedia passages and corresponding QA pairs - first training the model on the passages and later testing the amount of knowledge captured via the QA pairs. The experimental procedure is shown in Figure~\ref{fig:experimental_setup}.

% \mpara{Pretraining tasks.} While we show that all tasks result in the model retaining factual knowledge from the additional pretraining corpus, both average performance and variance vary from task to task. Our results suggest that SSM and PMI masking both outperform random token masking (61.1\%), with PMI masking having the least amount of variance between runs (72.0\% compared to others \%). 

% \mpara{Catastrophic forgetting of knowledge.} We show that the sequential learning problem also occurs with the current training paradigm of additional pretraining followed by closed-book question answering. This is in line with the findings of \citet{wallat-etal-2020-bertnesia}, who observed that fine-tuning leads to factual knowledge being forgotten.

% \mpara{Mitigation of catastrophic forgetting.} We find that common countermeasures to catastrophic forgetting can be applied to mitigate the effect of knowledge no longer being accessible. Multi-task learning seems to be slightly more effective than elastic weight consolidation (EWC), yet both result in significant performance improvement over the baseline. Additionally, we find that MTL and EWC reduce the run performance variance by XYZ and WXY\%.

% \begin{enumerate}
%     \item Additional pre-training tasks have a important effect on the amount of knowledge captured
%     \item The sequential learning problem (catastrophic forgetting [in a way]) is also existent with factual knowledge. In accordance with \citet{wallat}. 
%     \item Common counters to catastrophic forgetting also counter the forgetting of factual knowledge. (Elastic weight consolidation, multi-task learning).
%     \item While there is a large amount of variance in the amount of knowledge trained after additional pre-trianing (on all tasks but SSM the most), we observe MTL and EWC to highly reduce the variance in performance. 
% \end{enumerate}

==> chapters/intro.tex <==
\section{Introduction}


% What
Over recent years, overparameterized language models (LMs) such as BERT~\citep{DBLP:conf/naacl/DevlinCLT19} or T5~\citep{DBLP:journals/jmlr/RaffelSRLNMZLL20} have been increasingly applied to knowledge intensive tasks~\citep{DBLP:conf/naacl/PetroniPFLYCTJK21}; question answering, fact checking, and ranking to name only a few. One thing that makes these models so successfull is that their large parameter space allows them to learn syntactic, semantinc~\citep{DBLP:conf/acl/TenneyDP19} and factual~\citep{DBLP:conf/emnlp/PetroniRRLBWM19} knowledge from their training data. 

% Why
A better grasp of how knowledge is acquired and retained for downstream tasks could yield two major benefits: First, it will allow us to build more knowledgeable models, enabling better task performance. Second, it will be an early step in understanding when and under which circumstances unwanted or biased knowledge might be retained, potentially allowing us to later build more robust, socially responsible models. Studying how this factual knowledge is learned by language models is the main goal of this work.

% Probing and why we do CBQA 
A common approach to understanding the information picked up by latent models is probing the models for specific abilities \citep{DBLP:journals/corr/abs-2102-12452}. This usually entails training small classifiers on the LM's representations to predict linguistic properties such as part-of-speech tags \citep{DBLP:conf/acl/TenneyDP19}. However, probing allows for investigating if some property can be decoded from the model's embeddings - if and how the model utilizes these properties during inference is unclear \citep{DBLP:conf/eacl/RavichanderBH21}.
Therefore, we devise a different approach to understand the knowledge captured and retained from training: the model's ability to answer factual questions directly from its parametric memory. This setting, often referred to as closed-book question answering (CBQA) \citep{DBLP:conf/nips/LewisPPPKGKLYR020}, is a special case of the common open-domain question answering where no context or knowledge source can be used to produce an answer.
% This is a special subsetting of open-domain question \citep{cite} answering called closed-book question answering (CBQA) , where no additional context or knowledge source is allowed to answer the prompted questions - forcing the model to retrieve answers from its parameters. 
In contrast to the probing paradigm, improved CBQA performance can show that the model acquired additional knowledge \textit{and} its usability in downstream tasks.

% More details on CBQA and our setup
Recent works by \citet{DBLP:conf/emnlp/RobertsRS20} and \citet{DBLP:journals/corr/LewisPAQ} used an additional round of pretraining to infuse more knowledge into CBQA models. In this stage, models are trained on general knowledge sources (e.g., Wikipedia, C4) \citep{DBLP:journals/corr/LewisPAQ, DBLP:conf/emnlp/RobertsRS20} or additional context is retrieved during training \citep{DBLP:journals/corr/GuuREALM}.
% Limitations
While other studies applied additional pretraining to improve CBQA performance, no systematic analysis of additional pretraining, its tasks, and paradigms has been conducted. This is the goal of this work.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.49\textwidth]{figures/knowledge_pt_method_larger.pdf}
%     \caption{Experimental setup. First the model is additionally pretrained on knowledge-intense passages from Wikipedia, then it is trained on closed-book question answering and tested to measure the amount of knowledge retained.}
%     \label{fig:experimental_setup}
% \end{figure}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=0.8\textwidth]{figures/knowledge_pt_method_wide.drawio.pdf}
    \caption{Experimental setup. First the model is additionally pretrained on knowledge-intense passages from Wikipedia, then it is trained on closed-book question answering and finally tested on QA pairs directly build from the pretraining passages to measure the amount of knowledge retained.}
    \label{fig:experimental_setup}
\end{figure*}

% Our solution/idea
To understand how knowledge is retained from the additional pretraining stage and applied in CBQA, we leverage the PAQ dataset \citep{DBLP:journals/corr/LewisPAQ} which contains Wikipedia passages and multiple question-answer pairs directly extracted from each passage. This direct relation between a pretraining corpus and CBQA dataset allows for a systematic investigation of different pretraining tasks and their effect on the amount of factual knowledge being retained. To do so, we devise a three-step process (see Figure~\ref{fig:experimental_setup}): Firstly, a T5 model is additionally pretrained on the PAQ Wikipedia passages to capture relevant knowledge. Secondly, the model is trained for CBQA on a subset of the aligned QA pairs and lastly, we measure the amount of factual knowledge retained from training on a hold-out CBQA test set. We experiment with span corruption (RTM, random token masking - T5's version of language modeling) \citep{DBLP:journals/jmlr/RaffelSRLNMZLL20}, salient span masking (SSM, masking entities) \citep{DBLP:conf/acl/ZhangHLJSL19}, and PMI masking (masking by the pointwise mutual information of sequences) \citep{DBLP:conf/iclr/LevineLLALTS21}. 



% Experiments and some highlight results
% While we find that all additional pretraining tasks improve the amount of knowledge captured, SSM and PMI masking seem to be more effective than masking random tokens. Furthermore, our experiments suggest that catastrophic forgetting also occurs with factual knowledge and that these effects can be mitigated by regularization strategies such as elastic weight consolidation (EWC) \citep{DBLP:journals/corr/KirkpatrickPRVD16} or multi-task learning (MTL). 

% Contributions
\subsection{Contributions}
% Our research question and how it is novel
The fact that language models acquire factual knowledge from their pretraining is widely accepted and utilized for applying LMs to knowledge intensive tasks. Yet, it is poorly understood how and which knowledge is retained from training. Therefore, we pose two research questions: RQ1: \textit{"What is the effect of pretraining tasks on the amount of knowledge being acquired?"} and RQ2: \textit{"Is this knowledge still usable after fine-tuning for downstream tasks?"}


% Our approach
This study aims to improve our understanding of the parametric memory, by systematically studying the effect of additional pretraining tasks on the amount of factual knowledge captured and retained by the model. We utilize Wikipedia passages and corresponding QA pairs to first training the model on the passages and later testing the amount of knowledge captured via the QA pairs (see Figure~\ref{fig:experimental_setup}). Our key findings summarize as follows:

\mpara{Pretraining tasks.} While we show that all tasks result in the model retaining factual knowledge from the additional pretraining corpus, both average performance and variance vary from task to task. Our results suggest that SSM and PMI masking both outperform random token masking (61.1\%), with PMI masking having the least amount of variance between runs (72.0\% compared to others \%). 

\mpara{Catastrophic forgetting of knowledge.} We show that the sequential learning problem also occurs with the current training paradigm of additional pretraining followed by closed-book question answering. This is in line with the findings of \citet{wallat-etal-2020-bertnesia}, who observed that fine-tuning leads to factual knowledge being forgotten.

\mpara{Mitigation of catastrophic forgetting.} We find that common countermeasures to catastrophic forgetting can be applied to mitigate the effect of knowledge no longer being accessible. Multi-task learning seems to be slightly more effective than elastic weight consolidation (EWC), yet both result in significant performance improvement over the baseline. Additionally, we find that MTL and EWC reduce the run performance variance by XYZ and WXY\%.

% Key findings

% To improve our understanding of the parametric memory, we systematically study the effect of additional pretraining tasks on the amount of factual knowledge captured and retained by the model. Therefore, we utilize knowledge-dense Wikipedia passages and corresponding QA pairs - first training the model on the passages and later testing the amount of knowledge captured via the QA pairs. The experimental procedure is shown in Figure~\ref{fig:experimental_setup}.

% \mpara{Pretraining tasks.} While we show that all tasks result in the model retaining factual knowledge from the additional pretraining corpus, both average performance and variance vary from task to task. Our results suggest that SSM and PMI masking both outperform random token masking (61.1\%), with PMI masking having the least amount of variance between runs (72.0\% compared to others \%). 

% \mpara{Catastrophic forgetting of knowledge.} We show that the sequential learning problem also occurs with the current training paradigm of additional pretraining followed by closed-book question answering. This is in line with the findings of \citet{wallat-etal-2020-bertnesia}, who observed that fine-tuning leads to factual knowledge being forgotten.

% \mpara{Mitigation of catastrophic forgetting.} We find that common countermeasures to catastrophic forgetting can be applied to mitigate the effect of knowledge no longer being accessible. Multi-task learning seems to be slightly more effective than elastic weight consolidation (EWC), yet both result in significant performance improvement over the baseline. Additionally, we find that MTL and EWC reduce the run performance variance by XYZ and WXY\%.

% \begin{enumerate}
%     \item Additional pre-training tasks have a important effect on the amount of knowledge captured
%     \item The sequential learning problem (catastrophic forgetting [in a way]) is also existent with factual knowledge. In accordance with \citet{wallat}. 
%     \item Common counters to catastrophic forgetting also counter the forgetting of factual knowledge. (Elastic weight consolidation, multi-task learning).
%     \item While there is a large amount of variance in the amount of knowledge trained after additional pre-trianing (on all tasks but SSM the most), we observe MTL and EWC to highly reduce the variance in performance. 
% \end{enumerate}

==> chapters/results_old.tex <==
% \section{Results}

% Given the previously established methodology and data, we report our findings in this section. 

% \mpara{Random masking is least effective for retaining knowledge.}

% First, we experiment with the three different masking strategies on the PAQ dataset. For our experiments, we followed the methodology depicted in Figure~\ref{fig:experimental_setup}: Pretraining on the PAQ Wikipedia passages with one of our three pretraining tasks, followed by CBQA fine-tuning on the training set of corresponding QA pairs. Lastly, we measure the amount of knowledge retained from pretraining by the difference to a baseline model that was not additionally pretrained. We repeat all experiments four times.
% The results are reported in Figure~\ref{fig:pt_standard_setting}. First of all, we find the process of additional pretraining to improve the amount of knowledge retained for the downstream task, no matter of the specific masking strategy. This is in line with other works, reporting that additional pretraining improves the CBQA performance \citep{DBLP:journals/corr/GuuREALM, DBLP:conf/emnlp/RobertsRS20, DBLP:journals/corr/LewisPAQ}. Next, we observe PMI masking and SSM to outperform masking random tokens. We hypothize that this is the case, because RTM results in many easy to guess examples being masked (see Section~\ref{sec:infusing_knowledge}). Facts - or relational knowledge - are often expressed in the interactions and context of entities. However, with masking easy-to-guess examples, the model is never required to understand the broader context in which entities appear. Last, while we find the average performance of SSM and PMI to be fairly similar, we observe less variance in PMI masking compared to SSM or RTM.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/tmp/standard.png}
%     \caption{CBQA performance in F1 score for the baseline without additional pretraining (FT) and three models with additional pretraining and different masking strategies (RTM, SSM, PMI masking).}
%     \label{fig:pt_standard_setting}
% \end{figure}

% % \begin{figure}[h!]
% %     \centering
% %     \includegraphics[width=0.34\textwidth]{updated_plots/bert/multi_mean_P_AT_1.png}
% %     \caption{Mean P@1 of \bert{} across all layers.}
% %     \label{fig:bert_layers}
% % \end{figure}

% \mpara{The sequential learning problem applies to factual knowledge.}
% % Show that catastrophic forgetting is a problem

% Interestingly, the additional pretraining step on knowledge-rich textual data usually leads to small improvements in CBQA performance - typically a few percent in F1 or exact match \citep{DBLP:journals/corr/LewisPAQ, DBLP:journals/corr/GuuREALM}. This is what we observe in Figure~\ref{fig:pt_standard_setting}, despite a intensive additional pretraining stage on passages that we can be sure to contain the factual information (other than REALM, which tries to retrieve useful information from a corpus \citep{DBLP:journals/corr/GuuREALM}). Thus, we wonder if the sequential learning problem (also referred to as catastrophic forgetting) applies to factual knowledge being stored in the model's parametric memory. 
% % Short description of what I call catastrophic forgetting in this setting
% The classical sequential learning problems occurs when a model is trained on an initial task, fine-tuned on another and required to perform the initial again. In this szenario, many works have shown that the model is likely to lose parts of its ability to perform the initial task (\cite{CF}). Here, we hypothize that this also applies to (factual) knowledge acquired with the first task (might also partially explain why ft models were performing bad in knowledge tasks in \citep{wallat-etal-2020-bertnesia}). Therefore, we will experiment with common approaches to counter the sequential learning problem.  

% % 

% \mpara{Elastic Weight Consolidation.}

% In a first set of experiments, we additionally pretrained our models with the three tasks as before, but use the elastic weight consolidation (EWC, \citep{DBLP:journals/corr/KirkpatrickPRVD16}) regularizer in the fine-tuning stage. As EWC tries to preserve weights that are important for the initial task, it might also preserve the world knowledge acquired with this task. 

% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=0.45\textwidth]{figures/ewc.png}
% %     \caption{F1 Score comparing the training w/o EWC and /w EWC.}
% %     \label{fig:pt_ewc}
% % \end{figure}

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/tmp/ewc_mtl.png}
%     \caption{F1 Score comparing the training with EWC/MTL to the standard pretraining and fine-tuning setup.}
%     \label{fig:pt_ewc}
% \end{figure}

% Figure~\ref{fig:pt_ewc} compares the F1 scores achieved with the pretraining tasks with and without EWC. It it directly evident, that the amount of knowledge being retained and usable from the pretraining stage is vastly increased with the usage of EWC. This suggests, that the problem of catastrophic forgetting indeed applies to the knowledge captured with an initial task. In these experiments with EWC, we again find SSM and PMI masking to outperform RTM. However, the differences between the masking strategies are not as striking as in the standard setting. Additionally, a benefit of EWC is a reduced amount of varience between runs with the same masking strategy.  



% \mpara{Multi-task Learning.}

% Given the success of EWC to counter the forgetting of factual knowledge, we next experiment with multi-task learning. MTL has been shown to work well when it comes to retaining the ability to perform multiple tasks (\cite{MTL}). By not training two tasks sequentially, MTL forces to model to keep the ability to perform well in both tasks at the same time. Thus, we compare our standard setup to two different training strategies: Multi-task training both the additional pretraining and the CBQA fine-tuning together as well as the aforementioned Multi-task setup, followed by an additional CBQA fine-tuning step. The results are shown in Figure~\ref{fig:pt_multitask}.

% \begin{figure}[h]
%     \centering
%     \includegraphics[width=0.45\textwidth]{figures/multitask.png}
%     \caption{F1 for the multitask setting.}
%     \label{fig:pt_multitask}
% \end{figure}

% Similar to EWC, we find MTL to outperform the common setting of additional pretraining followed by CBQA fine-tuning. The standard MTL setup performs similar to EWC, however these results can be further improved by another round of fine-tuning. With this additional round of fine-tuning, we also observe the least amount of performance variance.


==> chapters/setup-avi.tex <==
\section{Knowledge Infusion Tasks}
\label{sec:kit}

To infuse knowledge and test retention, we follow the methodology depicted in Figure~\ref{fig:experimental_setup}: Pre-training on the passages with one of our three pre-training tasks (Section~\ref{sec:infusing_knowledge}), followed by CBQA fine-tuning on the training set of corresponding QA pairs. Lastly, we measure the amount of knowledge retained from pre-training by the difference to a baseline model that was not additionally pre-trained. All experiments are repeated four times. To keep our experiments tractable, we use T5-small with a total of 12 layers.

\subsection{Additional Pre-training}
\label{sec:infusing_knowledge}
To infuse knowledge into the model, we continue pre-training T5 on the language modeling objective.  
We use cross-entropy as our knowledge infusion loss (Formular~\ref{formula:loss}) with a batch size of 32 and a maximum number of 100 epochs (with early-stopping). 
We experiment with the following masking strategies:

\mpara{Random token masking.} In the RTM task, we apply the standard T5 language modeling task of span corruption. We randomly select positions and mask 15\% tokens or spans. We follow the details described in the original T5 paper \citep{DBLP:journals/jmlr/RaffelSRLNMZLL20}. 

\mpara{Salient span masking.} Instead of random tokens, salient span masking prioritizes masking named entities \citep{DBLP:conf/acl/ZhangHLJSL19}. As the answers in QA are mostly related to entities (e.g., "Who is the current French president?"), salient span masking could have a positive inductive bias by putting additional focus on entities. In our experiments we mask 15\% of the tokens. In case there are less entites in the sequence, we mask all available entities and default back to masking tokens randomly until we reach 15\% masked tokens. We used a BERT-base named entity recognizer \citep{DBLP:journals/corr/GuuREALM, DBLP:conf/emnlp/RobertsRS20}.  


\mpara{PMI masking.} The last of the masking strategies is masking by pointwise mutual information, proposed by  \citet{DBLP:conf/iclr/LevineLLALTS21}. The authors find that LMs can perform well in the RTM objective by abusing local features instead of understanding the general context. Therefore, they propose jointly masking n-grams with frequent collocation in the training corpus \citep{DBLP:conf/iclr/LevineLLALTS21}. We hypothesize two benefits of PMI masking for acquiring knowledge: The likelihood of masking non-informative tokens decreases (tokenizing "by the way" as one instead of 3 tokens) and the context of entities has to be understood (masking "the united states" as one token will not allow the easy guess of "the united [MASK]" -> states).


\subsection{CBQA Fine-tuning}

Before measuring how much knowledge is retained by the model, we fine-tune T5 for CBQA, allowing the model to learn how to answer questions. Therefore, we split our QA pairs into a training set and a holdout test set. As T5 models all tasks as sequence-to-sequence problems, the fine-tuning uses the cross-entropy loss (similar to knowledge infusion): 
\begin{equation}
    \mathcal{L}_{QA}= \mathcal{L}_{KI} =-\sum_{i=1}^{|V|}y_{i}log(p_i)
    \label{formula:loss}
\end{equation}
with the vocabulary size $|V|$ and the softmax probability of the individual tokens as $p_i$. For the CBQA fine-tuning, we use a batch size of 128 and train for a maximum of 100 epochs (with early stopping). At inference time, we generate answers using beamsearch decoding with five beams.  

After fine-tuning, we use the hold-out test set of QA pairs to test how much knowledge is retained. We measure the CBQA performance of the different knowledge-infused models and a baseline without additional pre-training and report F1 scores and exact match. If a model, after being pre-trained on the passages, improves in performance over the baseline, we say it acquired and retained knowledge from the pre-training process. We repeat all experiments four times.

\subsection{Data}
We use the PAQ dataset \citep{DBLP:journals/corr/LewisPAQ} for our experiments. This dataset contains a set of 65M QA pairs automatically generated from Wikipedia passages, with each passage having 4-8 QA pairs. Since the QA pairs are derived from a passage, we can be sure that the question's answer can be found in the said passage. Another benefit is that our QA pairs cover multiple facts in one passage, allowing for more precise measurements of what is retained. To keep our experiments tractable, we select 10K passages from the full PAQ dataset. For the additional pre-training, we utilize the full 10K passages. For the CBQA training, we split the ~49k QA pairs into train (76\%), dev (10\%), and test sets (14\%). 

